A Data-Driven McMillan Degree Lower Bound

Given measurements of a linear time-invariant system, the McMillan degree is the dimension of the smallest such system that reproduces these observed dynamics. Using impulse response measurements where the system has been started in some (unknown) state and then allowed to evolve freely, a classical result by Ho and Kalman reveals the McMillan degree as the rank of a Hankel matrix built from these measurements. However, if measurements are contaminated by noise, this Hankel matrix will almost surely be full rank. Hence practitioners often estimate the rank of this matrix---and thus the McMillan degree---by manually setting a threshold between the large singular values that correspond to the non-zero singular values of the noise-free Hankel matrix and the small singular values that are pertubations of the zero singular values. Here we introduce a probabilistic upper bound on the perturbation of the singular values of this Hankel matrix when measurements are corrupted by additive Gaussian noise, and hence provide guidance on setting the threshold to obtain a lower bound on the McMillan degree. This result is powered by a new, probabilistic bound on the 2-norm of a random Hankel matrix with normally distributed entries. Unlike existing results for random Hankel matrices, this bound features no unknown constants and, moreover, is within a small factor of the empirically observed bound when entries are independent and identically distributed. This bound on the McMillan degree provides an inexpensive alternative to more general model order selection techniques such as the Akaike Information Criteria (AIC).

==> abstract.tex <==
\begin{abstract}
% Background
In the context of linear time-invariant systems,
the McMillan degree prescribes the smallest possible dimension
of a system that reproduces the observed dynamics.
When these observations take the form of impulse response measurements
where the system evolves without input from an unknown initial condition,
a result of Ho and Kalman reveals the McMillan degree 
as the rank of a Hankel matrix built from these measurements.
% The problem: noise
Unfortunately using this result in experimental practice is challenging
as measurements are invariably contaminated by noise
and hence the Hankel matrix will almost surely be full rank.
Hence practitioners estimate the rank of this matrix---and thus the McMillan degree---%
by manually setting a threshold separating  
large singular values corresponding to the non-zero singular values of the noise-free Hankel matrix
and small singular values corresponding to perturbation of zero singular values of the noise-free Hankel matrix. 
% Our contribution
Here we replace this manual threshold 
with a threshold guided by Weyl's theorem.
Specifically, assuming measurements are perturbed by additive Gaussian noise
we construct a probabilistic upper bound
on how much the singular values of the noise-free Hankel matrix can be perturbed;
this provides a conservative threshold for estimating the rank, and hence the McMillan degree.
% lemma on 2-norm
This result follows from a new probabilistic bound on the 2-norm 
of a random Hankel matrix with normally distributed entries. 
% Comparison to background
Unlike existing results for random Hankel matrices, 
this bound features no unknown constants
and, moreover, is within a small factor of the empirically observed bound.
% Relation to model selection criteria from statistics
This bound on the McMillan degree provides an inexpensive alternative to more general
model order selection techniques such as the Akaike Information Criteria (AIC).
\end{abstract}

